The Limits to Learning a Diffusion Model

This paper provides the first sample complexity lower bounds for the estimation of simple diffusion models, including the Bass model (used in modeling consumer adoption) and the SIR model (used in modeling epidemics). We show that one cannot hope to learn such models until quite late in the diffusion. Specifically, we show that the time required to collect a number of observations that exceeds our sample complexity lower bounds is large. For Bass models with low innovation rates, our results imply that one cannot hope to predict the eventual number of adopting customers until one is at least two-thirds of the way to the time at which the rate of new adopters is at its peak. In a similar vein, our results imply that in the case of an SIR model, one cannot hope to predict the eventual number of infections until one is approximately two-thirds of the way to the time at which the infection rate has peaked. This lower bound in estimation further translates into a lower bound in regret for decision-making in epidemic interventions. Our results formalize the challenge of accurate forecasting and highlight the importance of incorporating additional data sources. To this end, we analyze the benefit of a seroprevalence study in an epidemic, where we characterize the size of the study needed to improve SIR model estimation. Extensive empirical analyses on product adoption and epidemic data support our theoretical findings.

==> sections/Tianyi_results.tex <==
%!TEX root=../SIR-model-EC.tex
\section{Tianyi Results}

Let $t_1 = \inf\{I(t) \geq N^{2/3}\}, t_2 = \inf\{I(t) \geq \mathring{m}\}$ where $\mathring{m} = \min\left\{k\geq 1~|~\bE[T_{k}] \geq \bE[T_{k-1}]\right\}.$ Hence $t_2$ is the time when the increasing rate of $I(t)$ achieves the maximum. A quick calculation can show that $\mathring{m} = \left\lceil\frac{(1-\frac{p}{\beta})N+1}{2}\right\rceil.$

\begin{proposition}
Suppose $\gamma = 0, I_0= 1, \frac{p}{\beta} < c$ for some constant $c < 1$. Suppose $\frac{p}{\beta} = \Theta(\frac{1}{N^{\alpha}})$.
\begin{align}
\lim_{N \rightarrow \infty} \frac{\bE[t_1]}{\bE[t_2]} =
\begin{cases}
0 & \alpha \leq \frac{1}{3}\\
\frac{\alpha - \frac{1}{3}}{\alpha} & \frac{1}{3} < \alpha \leq 1\\
\frac{2}{3} &  1<\alpha
\end{cases}
\end{align}
\end{proposition}

\begin{proof}
Note that $\bE[T_{i}] = \frac{N}{pN(N-i) + \beta i (N-i)}.$ Then 
$$
\bE[t_1] = \bE\left[\sum_{i=1}^{N^{2/3}-1} T_{i}\right] = \sum_{i=1}^{N^{2/3}-1} \frac{N}{pN(N-i) + \beta i (N-i)}.
$$
Let $f(x) = \frac{N}{pN(N-x) + \beta x (N-x)}$, we use $f(x)$ as a proxy to bound $\bE[t_1].$ Easy to verify that $f(x)$ is decreasing when $x \in (0, \mathring{r}]$ where $\mathring{r} = (1-p/\beta)N/2.$  Note that $p/\beta < c$ for some constant $c$. Hence when $N \rightarrow \infty$, we have $\mathring{r} \gg N^{2/3}$ and
\begin{align*}
\sum_{i=1}^{N^{2/3}-1} \frac{N}{pN(N-i) + \beta i (N-i)} 
&\geq \int_{x=1}^{N^{2/3}} f(x)dx\\
&= \frac{\ln (\beta x + Np) - \ln (N-x)}{p+\beta} \Big\rvert_{x=1}^{N^{2/3}}\\
&= \frac{\ln (\beta N^{2/3} + Np) - \ln (\beta + Np) + \ln (N-1) - \ln (N - N^{2/3})}{p + \beta}\\
&\geq \frac{\ln (\beta N^{2/3} + Np) - \ln (\beta + Np)}{p + \beta}.
\end{align*}

Similarly, for $t_2$, we have
\begin{align*}
E[t_2] &= \sum_{i=1}^{\mathring{m}-1} \frac{N}{pN(N-i) + \beta i (N-i)} \\
&\leq f(1) + \int_{x=1}^{\mathring{r}} f(x)dx\\
&\leq f(1) + \frac{\ln (\beta N + Np) - \ln (pN + \beta) + \ln \frac{1}{1-c}}{p + \beta}\\
&\leq \frac{\ln (\beta N + Np) - \ln (pN + \beta) + c'}{p + \beta}
\end{align*}
for some absolute constant $c'$.

Let $\frac{\beta}{p} = C\cdot N^{\alpha}$ for some constant $C.$ We then have
\begin{align*}
\frac{E[t_1]}{E[t_2]} 
&\geq  \frac{\ln (\beta N^{2/3} + Np) - \ln (\beta + Np)}{\ln (\beta N + p N) - \ln (pN+\beta) + c'}\\
&\geq \frac{\ln\left(\frac{CN^{2/3+\alpha} + N}{CN^{\alpha} + N} \right)}{\ln\left(\frac{CN^{1+\alpha} + N}{CN^{\alpha} + N} \right) + c'} =: k_{N}.
\end{align*}

Then, it is easy to verify that when $ \frac{1}{3} <\alpha \leq 1$, $\lim_{N\rightarrow \infty} k_{N} = \frac{\alpha-1/3}{\alpha}.$ When $\alpha 
> 1$, $\lim_{N\rightarrow \infty} k_{N} = \frac{2}{3}.$ 

Note that we also have $\bE[t_1] \leq f(1) + \int_{x=1}^{N^{2/3}} f(x)dx$ and $\bE[t_2] \geq \int_{x=1}^{\mathring{r}} f(x)dx$. Similarly, one can verify that
\begin{align*}
\limsup_{N\rightarrow \infty} \frac{\bE[t_1]}{\bE[t_2]} \leq  \begin{cases} 0 & \alpha \leq \frac{1}{3} \\ \frac{\alpha - \frac{1}{3}}{\alpha} & \frac{1}{3} <\alpha \leq 1 \\ \frac{2}{3} & \alpha > 1\end{cases}.
\end{align*}
This completes the proof. 
\end{proof}




\begin{table}
\centering
\begin{tabular}{@{}cccc@{}}
\toprule
&$ \relerror(\hat{N}, N)$ & $\relerror(\hat{a}, a) $& $\relerror(\hat{\beta}, \beta)$ \\%& Anomaly Detection rate \\
\midrule
$\frac{p}{\beta} = \Theta(\frac{1}{N^{\alpha}})$ & $O\left(\frac{N^2}{m^3}\right)$ & $\tilde{O}\left(\frac{1}{m} +\frac{1}{N^{(1-\alpha)}}\right)$ &$\tilde{O}\left(\frac{1}{m} + \frac{N^{2(1-\alpha)}}{m^3}\right)$ \\%&--\\ 
%$\frac{1}{3} <\alpha \leq 1$ & $O\left(\frac{N^2}{m^3}\right)$ & -- \\
%$1 < \alpha$ & $O\left(\frac{N^2}{m^3}\right)$ & -- \\%& --\\
\bottomrule
\end{tabular}
\caption{The relative error of estimating $(N, a, \beta)$ where $a=pN$ in Bass model. $m$ is the number of samples.}
\end{table}


\begin{table}
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
&$ \relerror(\hat{N}, N)$ & $\relerror(\hat{a}, a) $& $\relerror(\hat{\beta}, \beta)$ & $\frac{\bE[t_1]}{\bE[t_2]}$ \\%& Anomaly Detection rate \\
\midrule
$0\leq \alpha \leq \frac{1}{3}$ & $O(1)$ & $\tilde{O}\left(\frac{1}{N^{2/3}}\right)$ &$\tilde{O}\left(\frac{1}{N^{2\alpha}}\right)$ & $0$\\%&--\\ 
$\frac{1}{3} <\alpha \leq 1$ & $O(1)$ & $\tilde{O}\left(\frac{1}{N^{1-\alpha}}\right)$ & $\tilde{O}\left(\frac{1}{N^{2/3}}\right)$ & $\frac{\alpha-\frac{1}{3}}{\alpha}$\\
$1 < \alpha$ & $O(1)$ & - & $\tilde{O}\left(\frac{1}{N^{2/3}}\right)$ & $\frac{2}{3}$\\%& --\\
\bottomrule
\end{tabular}
\caption{The relative error of estimating $(N, a, \beta)$ in Bass model when $N^{2/3}$ samples are observed. $\frac{\bE[t_1]}{\bE[t_2]}$ is the ratio between the time for observing $N^{2/3}$ samples and the peak time. }
\end{table}

\begin{theorem}
Suppose $\gamma = 0, I_0 = 1$. Let $a = pN.$ Suppose $m \leq N^{2/3}\log^{1/3}(N)$. There exists estimator $\hat{a}, \hat{\beta}$ such that with probability $1-O(\frac{1}{N})$, 
\begin{align*}
\relerror(\hat{\beta}, \beta) = O\left(\frac{\log N}{m} + \frac{a^2}{\beta^2}\frac{\log N}{m^3} \right)\\
\relerror(\hat{a}, a) = O\left(\frac{\log N}{m} + \frac{\beta}{a} \log N\right).
\end{align*}
\end{theorem}


\begin{proof}
For simplicity, assume $m = 2k.$ Let $A_i = \min(T_i, T_{m-i}), 1\leq i \leq k$. It is easy to see that $A_i \sim \mathrm{Exp}(l_i)$
where
$$
l_i := (2a + \beta m)-(a + i\beta)\frac{i}{N} - (a + (m-i)\beta)\frac{m-i}{N}.
$$
Consider $S = \sum_{i=1}^{m/2} A_i.$ Then by Theorem 5.1 in \cite{janson2018tail}, for any $\delta > 0$
\begin{align*}
\Pr(S \geq (1+\delta)\mu) \leq e^{-l_{*}\mu(\delta-\ln(1+\delta))}
\end{align*}
where $\mu = E[S], l_{*} \leq \min_{i=1}^{m/2} l_i.$ It is easy to check that
\begin{align*}
\frac{N-m}{N} (2a + \beta m) \leq l_i \leq 2a+\beta m
\end{align*}

We can let $l_{*} = (2a+\beta m) \frac{N-m}{N}.$ Furthermore, we can also obtain bounds for $\mu = \sum_{i=1}^{m/2} \frac{1}{l_i}$:
\begin{align*}
\frac{1}{2}\frac{m}{2a+m\beta} \leq \mu \leq \frac{1}{2} \frac{N}{N-m}\frac{m}{2a+m\beta}.
\end{align*}

Take $\delta = O(\sqrt{\frac{\log(N)}{m}}).$ Note that $\delta - \ln(1+\delta) = O(\frac{\log(N)}{m}).$ We will have
\begin{align*}
\Pr(\frac{S}{m} \geq (1+\delta)\frac{\mu}{m}) \leq e^{-l_{*}\mu(\delta-\ln(1+\delta))} = e^{-\frac{(N-m)m}{N} O(\frac{\log(N)}{m})} = O(\frac{1}{N^2})
\end{align*}
using the assumption $\frac{N-m}{N} \geq \frac{1}{2}$. Similar bounds can be obtained for the lower bound. Then one can verify that, with probability $1-O(1/N^2)$, we have, for some constant $C_1$
\begin{align*}
\left|\frac{m}{2S} - \left(2a + m\beta\right)\right| 
&\leq C_1\left(\min(2a+m\beta, m/2S)\left(\frac{m}{N} + \sqrt{\frac{\log(N)}{m}}\right)\right)\\
&\leq C_1(a \sqrt{\frac{\log(N)}{m}} + \sqrt{m}\beta \sqrt{\log(N)}).
\end{align*}
Similarly, let $S' = \sum_{i=1}^{m/4} min(T_{i}, T_{m/2-i}).$ One can verify that with probability $1-O(1/N^2)$, 
\begin{align*}
\left|\frac{m}{4S'} - \left(2a + \frac{m}{2}\beta\right)\right| \leq C_1 (a \sqrt{\frac{\log(N)}{m}} + \sqrt{m}\beta \sqrt{\log(N)}).
\end{align*}
One can verify for any $\hat{\alpha}, \hat{\beta}$ satisfy the following inequality
\begin{align*}
\left|\frac{m}{2S} - \left(2\hat{a} + m\hat{\beta}\right)\right| \leq C_1\left(\frac{m}{2S}\left(\frac{m}{N} + \sqrt{\frac{\log(N)}{m}}\right)\right)\\
\left|\frac{m}{4S'} - \left(2\hat{a} + \frac{m}{2}\hat{\beta}\right)\right| \leq C_1\left(\frac{m}{4S'}\left(\frac{m}{N} + \sqrt{\frac{\log(N)}{m}}\right)\right)
\end{align*}
we will have
\begin{align*}
|\hat{\beta}-\beta| &= O\left(a \sqrt{\frac{\log(N)}{m^3}} +  \beta \sqrt{\frac{\log(N)}{m}} \right)\\
|\hat{a} - a| &= O\left(a \sqrt{\frac{\log N}{m}} + \sqrt{m} \beta \sqrt{\log N}\right)
\end{align*}

In order to obtain the optimal estimators, we consider a union of estimators where $S_{k} = \sum_{i=1}^{k/2} \min(T_{i}, T_{k-i}).$ We find the estimator $\hat{\alpha}, \hat{\beta}$ such that for every $k$,
\begin{align*}
\left|\frac{k}{2S} - \left(2\hat{a} + k\hat{\beta}\right)\right| \leq C_1\left(\frac{k}{2S}\left(\frac{m}{N} + \sqrt{\frac{\log(N)}{m}}\right)\right).
\end{align*}
This will guarantee, with probability $1-O(1/N)$, 
\begin{align*}
|\hat{\beta}-\beta| &= O\left(a \sqrt{\frac{\log(N)}{m^3}} +  \beta \sqrt{\frac{\log(N)}{m}} \right)\\
|\hat{a} - a| &= O\left(\min_{1\leq k\leq m} \left(a \sqrt{\frac{\log N}{k}} + \sqrt{k} \beta \sqrt{\log N}\right)\right) = O\left(a \sqrt{\frac{\log N}{m}} + \sqrt{\beta a} \sqrt{\log N}\right)
\end{align*}
\end{proof}





==> sections/extended_abstract_text.tex <==
This paper provides the first sample complexity lower bounds for the estimation of simple diffusion models which seek to explain the diffusion of an epidemic in a network. The Susceptible-Infected-Recovered (SIR) model is a classic example, proposed nearly a century ago [2]. The SIR model remains a cornerstone for the forecasting of epidemics. The so-called Bass model [1] remains a basic building block in forecasting consumer adoption of new products and services. The durability of these models arises from the fact that they have shown an excellent fit to data, in numerous studies spanning both the epidemiology and marketing literatures. Somewhat paradoxically, using these same models as reliable forecasting tools presents a challenge.

While we are ultimately motivated by the problem of forecasting a diffusion model, this paper asks a more basic question that is surprisingly unanswered: What are the limits to learning a diffusion model? We answer this question by characterizing sample complexity lower bounds for a class of stochastic diffusion models that encompass both the Bass model and the SIR model. We show that the time to collect a number of observations that exceeds these lower bounds is too large to allow for accurate forecasts early in the process.

In the context of the Bass model our results imply that when adoption is driven by imitation, one cannot hope to predict the eventual number of adopting customers until one is at least two-thirds of the way to the time at which the rate of new adopters is at its peak. In a similar vein, our results imply that in the case of an SIR model, one cannot hope to predict the eventual number of infections until one is approximately two-thirds of the way to the time at which the infection rate has peaked. Our analysis is conceptually simple and relies on the Cramer-Rao bound. The core technical difficulty in our analysis rests in characterizing the Fisher information in the observations available due to the fact that they have a non-trivial correlation structure.

 Maximum likelihood estimation of diffusion models on product adoption datasets (for products on Amazon.com), and epidemic data (from the ongoing COVID-19 epidemic) illustrate precisely the behavior predicted by our theory. As a byproduct of our analysis, we see that the difficulty in learning a diffusion model stems solely from uncertainty in a single unknown `effective population size' parameter. In particular, other parameters, including those related to the `rate of imitation' (in the Bass model) or the `reproduction number' (in the SIR model) are easy to learn. This suggests that estimators that rely on an (informative) bias in this population size parameter can in fact overcome the limitations presented by our analysis. Although not a primary contribution of the present work, we describe a heuristic procedure used to construct such a biased estimator that yielded one of the first US county-level forecasters available for COVID-19.

The full paper is available at https://arxiv.org/abs/2006.06373.

==> sections/graphical_model.tex <==

\begin{figure}
  \centering
  \centering
  \tikz{ %
    \node[obs] (I) {$O$} ; %
    \node[latent, above=of I] (beta) {$\beta$} ; %
    \node[obs, above=of beta] (X_d) {$M$} ; %
    \node[latent, left=of beta] (alpha) {$\alpha$} ; %
    \node[obs, above=of alpha] (X) {$X$} ; %
    \node[latent, below=of alpha] (N) {$N$} ; %
    \node[obs, left=of N] (P) {$P$} ; %
    \node[latent, right=of I] (gamma) {$\gamma$} ; %
    \plate[inner sep=0.25cm, xshift=-0.12cm, yshift=0.12cm] {plate1} {(beta) (I) (X_d)} {$m$}; %
    \plate[inner sep=0.25cm, xshift=-0.12cm, yshift=0.12cm] {plate2} {(alpha) (X) (P) (N) (plate1)} {$n$}; %
    \edge {gamma} {I} ; %
    \edge {beta} {I} ; %
    \edge {X_d} {beta} ; %
    \edge {X} {beta} ; %
    \edge {X} {alpha} ; %
    \edge {alpha} {N} ; %
    \edge {P} {N} ; %
    \edge {N} {I} ; %
  }
  \caption{
  Graphical diagram of the model. Shaded variables are observed, others are latent. 
  $n$ is the number of locations, and $m$ is the number of events.
  }
\end{figure}


% \begin{figure}
%   \centering
%   \tikz{ %
%     \node[obs] (I) {$O_{i,k}$} ; %
%     \node[latent, above=of I] (beta) {$\beta_{i,k}$} ; %
%     \node[obs, above=of beta] (X_d) {$X^d_{i,k}$} ; %
%     \node[latent, left=of beta] (alpha) {$\alpha_i$} ; %
%     \node[obs, above=of alpha] (X) {$X_i$} ; %
%     \node[latent, below=of alpha] (N) {$N_i$} ; %
%     \node[obs, left=of N] (P) {$P_i$} ; %
%     \node[latent, right=of I] (gamma) {$\gamma$} ; %
%     \plate[inner sep=0.25cm, xshift=-0.12cm, yshift=0.12cm] {plate1} {(beta) (I) (X_d)} {m}; %
%     \plate[inner sep=0.25cm, xshift=-0.12cm, yshift=0.12cm] {plate2} {(alpha) (X) (P) (N) (plate1)} {$i=1, \dots, n$}; %
%     \edge {gamma} {I} ; %
%     \edge {beta} {I} ; %
%     \edge {X_d} {beta} ; %
%     \edge {X} {beta} ; %
%     \edge {X} {alpha} ; %
%     \edge {alpha} {N} ; %
%     \edge {P} {N} ; %
%     \edge {N} {I} ; %
%   }
% \end{figure}

==> sections/proof_outline.tex <==
\subsection{Proof Outline}
We provide a proof sketch of Theorem~\ref{thm:fi}.

We first review several known properties of conditional Fisher information.
Let $g_{X|Y}(x, y, \theta) = \frac{\partial}{\partial \theta} \log f_{X|Y; \theta}(x|y)$ be the \textit{score} of the conditional distribution of $X$ given $Y=y$ with parameter $\theta$ evaluated at $x$.
Then, the conditional Fisher information is defined as
\begin{align*}
\cJ_{X|Y}(\theta)  = \bE_{X, Y}\left[g_{X| Y}(X, Y, \theta)^2\right].
\end{align*}
\begin{property} \label{property:chain_rule}
For random variables $X_1, \dots, X_n$,
  $\cJ_{X_1, \dots, X_n}(\theta) = \sum_{i = 1}^n \cJ_{X_i | X_1, \dots, X_{i-1}}(\theta)$.
\end{property}
\begin{property}  \label{property:indep}
  If $X$ is independent of $Z$ conditioned on $Y$, $\cJ_{X|Y,Z}(\theta) = \cJ_{X|Y}(\theta)$.
\end{property}
\begin{property} \label{property:deterministic}
% If $X$ is deterministic, $\cJ_{X}(\theta) = 0.$
If $X$ is deterministic given $Y=y$, $g_{X| Y}(X, y, \theta) = 0$.
\end{property}
% \begin{property}
% If $\theta$ is a continuously differentiable function of $\eta$, then $\cJ_{X}(\eta) = \cJ_{X}(\theta) \left(\frac{d \theta}{d \eta}\right)^2$.
% \end{property}

We use these properties in the following lemma to write a simple expression for $\cI_{O_m}(N)$.
\begin{lemma}  \label{lemma:fi}
The Fisher information of the observations $O_m$ with respect to the parameter $N$ is
\begin{align}
\cI_{O_m}(N)
&= \sum_{k=1}^{m} \Pr(E_{k-1}=1)  \bE\left[\frac{C_{k-1}^2}{N^2 (N-C_{k-1})((N-C_{k-1}) + \frac{\gamma}{\beta} N)} \bigg| E_{k-1} = 1 \right]. \label{eq:exactFI}
\end{align}
\end{lemma}
\begin{proof}[Proof sketch of Lemma~\ref{lemma:fi}.]
Since $O_m = (C_0, T_1, C_1, T_2, C_2, \dots, T_m, C_m)$, Property~\ref{property:chain_rule} implies
\begin{align*}
\cI_{O_m}(N) &= \cI_{C_0}(N)  + \cI_{T_1|C_0}(N) + \cI_{C_1|T_1,C_0}(N) + \cI_{T_2|C_1,T_1,C_0}(N) +  \cI_{C_2|T_2,C_1,T_1,C_0}(N) + \dots.
\end{align*}
$\cI_{C_0}(N)=0$  since $C_0$ is a known quantity.
Note that the distribution of the $k$-th jump (both the inter-arrival time and whether the jump corresponds to a new infection or recovery) only depends on the state of the system at the jump $k-1$.
That is, for any $k$, both $C_k$ and $T_k$ depend only on $C_{k-1}$.
Therefore, we can use Property~\ref{property:indep} to simplify the above equation to
\begin{align*}
\cI_{O_m}(N) &=\sum_{k=1}^m (\cJ_{C_k|C_{k-1}}(N) + \cJ_{T_k|C_{k-1}}(N)).
\end{align*}
If $E_{k-1}=0$ (the stopping time has passed), $C_k$ and $T_k$ are deterministic conditioned on $C_{k-1}$, which implies the
score in this case is 0 (Property~\ref{property:deterministic}).
Therefore, we can condition on $E_{k-1}=1$ to write
\begin{align*}
\cI_{O_m}(N)
&= \sum_{k=1}^m \bE[g_{C_k|C_{k-1}}(C_k,C_{k-1}, N) + g_{T_k|C_{k-1}}(T_k,C_{k-1}, N)| E_{k-1}=1] \Pr(E_{k-1}=1).
\end{align*}
When $E_{k-1}=1$, the distributions of $C_k$ and $T_k$ conditioned on $C_{k-1}$ have a simple form: they are Bernoulli and exponential distributions respectively with parameters that are functions of $\beta, \gamma, N$, and $C_{k-1}$.
Evaluating the score with these distributions results in the desired equation \eqref{eq:exactFI}.
\end{proof}

Given \eqref{eq:exactFI}, the upper bound $\cI_{O_m}(N) = O\left(\frac{m^3}{N^4}\right)$ can be easily derived using the fact that $\Pr(E_{k-1}) \leq 1$ and $C_{k} \leq k + I_0$.

For the lower bound, we first prove a lower bound for $\Pr(E_{m})$ provided in the next lemma.
Additionally, by using the definition of $k$, $C_k$, and $E_k$, it is not hard to see that $E_k = 1$ implies $C_k \geq \frac{k + I_0}{2}$.
Substituting these lower bounds for $\Pr(E_{m})$ and $C_k$ into \eqref{eq:exactFI} results in $\cI_{O_m}(N) = \Omega\left(\frac{m^3}{N^4}\right)$ as desired.
\begin{lemma} \label{lem:highprob}
There exists a constant $D$ (that depends only on $\beta$ and $\gamma$) such that
if $\eta(N, \beta, m+I_0) > p$ and $I_0 \geq D$,
then $\Pr(E_{m}) \geq \frac{1}{2}$.
\end{lemma}
% For the lower bound, we first show that $\Pr(E_{k-1}) \geq \frac{1}{2}$ given than the initial number of infections is larger than some constant $D$.
\begin{proof}[Proof sketch of Lemma~\ref{lem:highprob}]
We define another infection process with a slower rate of transmission than the SIR process of interest, and is also simpler to analyze.
Let $\{A_k\}_{k =0, 1, \dots}$ be a stochastic process with stopping time $\tau_A$. % , which we define similarly to the process $\{C_k\}_{k =0, 1, \dots}$.
% Recall that if the stopping time hasn't been reached by $k-1$ jumps, $C_k - C_{k-1}\sim  \Bern(\eta(N, \beta, \gamma, C_{k-1}))$.
$\{A_k\}_k$ is defined to have the same initial condition and stopping criterion as $\{C_k\}_k$, but before the stopping time, $A_k - A_{k-1} \sim \Bern(p)$ for a constant $p$, where $p < \frac{\beta S_{k-1}}{\beta S_{k-1} + N\gamma}$ for all $k < m$.
We show $\Pr(\tau < m) \leq \Pr(\tau_A < m)$ by proving that $A_k$ is stochastically less than $C_k$ for any $k$.
Since $A_k$ is a sum of i.i.d. Bernoulli random variables up to the stopping point, $\Pr(\tau_A < m)$ can be bounded using a Chernoff bound.
\end{proof}

\section{Alternate proof}

\subsection{Proof2 of Theorem~\ref{thm:fi}}

% Our goal is to show both upper and lower bounds for $\cI_{O_m}(N)$.
We first state three lemmas which are proven in the next section.
\begin{lemma} \label{lem:E_k}
Define $r_k \triangleq \frac{I_0 + k + 2R_0}{2}$ for all $k \geq 0$.
For all $k$, $E_k = \bI\{C_{k} > r_{k}\}$.
Moreover, when $E_k = 1$, $I_k = 2C_k - k - I_0 - 2R_0 > 0$.
% Moreover, $C_k$ determines $E_k$.
\end{lemma}

\begin{lemma}  \label{lemma:fi}
The Fisher information of the observations $O_m$ with respect to the parameter $N$ is
\begin{align}
\cI_{O_m}(N)
&= \sum_{k=1}^{m} \Pr(E_{k-1}=1)  \bE\left[\frac{C_{k-1}^2}{N^2 (N-C_{k-1})((N-C_{k-1}) + \frac{\gamma}{\beta} N)} \bigg| E_{k-1} = 1 \right]. \label{eq:exactFI}
\end{align}
\end{lemma}

\begin{lemma} \label{lem:highprob}
There exists a constant $D$ that only depends on $\beta$ and $\gamma$ such that if $\eta(N, \beta, m+I_0) > p$ and $I_0 \geq D$,
then $\Pr(E_{m}) \geq \frac{1}{2}$.
\end{lemma}

Theorem~\ref{thm:fi} follows readily from these lemmas.
Specifically, Lemma~\ref{lemma:fi} provides an exact expression for $\cI_{O_m}(N)$ that can be used for both the upper and lower bound.
For the lower bound, Lemma~\ref{lem:E_k} implies $C_k \geq \frac{k + I_0 + 2R_0}{2}$ when $E_k = 1$, and  Lemma~\ref{lem:highprob} implies $\Pr(E_k) \geq 1/2$. Substituting these bounds into \eqref{eq:exactFI} gives
\begin{align*}
\cI_{O_m}(N)
&\geq \frac{1}{2} \sum_{k=0}^{m-1}  \frac{(\frac{k+I_0}{2})^2}{N^3 (N + \frac{\gamma}{\beta} N)}.
\end{align*}
The lower bound $\cI_{O_m}(N) = \Omega(\frac{m^3}{N^4})$ follows from using $\sum_{k=1}^m k^2 = \Theta(m^3)$.
The upper bound $\cI_{O_m}(N) = O(\frac{m^3}{N^4})$ is found analogously using $C_k \leq k + I_0 + R_0 = o(N)$ and $\Pr(E_k) \leq 1$.

% this implies the numerator in the expectation in \eqref{eq:exactFI} is $\Theta(k^2)$.
% Moreover, since $m = o(N)$ and hence $C_k = o(N)$, the denominator of the expectation in \eqref{eq:exactFI} is $\Theta(N^4)$.
% Therefore,
% \begin{align}
% \cI_{O_m}(N)
% &= \sum_{k=1}^{m} \Pr(E_{k-1}=1) \Theta\left(\frac{k^2}{N^4}\right).
% \end{align}
% Lastly, using $1/2 \leq \Pr(E_k) \leq 1$ from Lemma~\ref{lem:E_k} and $\sum_{k=1}^m \Theta(k^2) = \Theta(m^2)$ proves the desired result.
Lemma~\ref{lem:E_k} follows from the definitions of $\tau$, $E_k$, and $C_k$; the details can be found in the appendix.
The rest of the section is dedicated to proving Lemmas~\ref{lemma:fi} and \ref{lem:highprob}.

\subsubsection{Background on Fisher Information}
First, we state several known properties of conditional Fisher information.
Let $g_{X|Y}(x, y, \theta) = \frac{\partial}{\partial \theta} \log f_{X|Y; \theta}(x|y)$ be the \textit{score} of the conditional distribution of $X$ given $Y=y$ with parameter $\theta$ evaluated at $x$.
Then, the conditional Fisher information is defined as
\begin{align*}
\cJ_{X|Y}(\theta)  = \bE_{X, Y}\left[g_{X| Y}(X, Y, \theta)^2\right].
\end{align*}
\begin{property} \label{property:chain_rule}
For random variables $X_1, \dots, X_n$,
  $\cJ_{X_1, \dots, X_n}(\theta) = \sum_{i = 1}^n \cJ_{X_i | X_1, \dots, X_{i-1}}(\theta)$.
\end{property}
\begin{property}  \label{property:indep}
  If $X$ is independent of $Z$ conditioned on $Y$, $\cJ_{X|Y,Z}(\theta) = \cJ_{X|Y}(\theta)$.
\end{property}
\begin{property} \label{property:deterministic}
If $X$ is deterministic given $Y=y$, $g_{X| Y}(X, y, \theta) = 0$.
\end{property}

\subsubsection{Proofs of Lemmas}
% Recall $E_k = \bI\{\tau > k\}$ is the indicator that the process has not terminated after $k$ jumps.

\begin{proof}[Proof of Lemma~\ref{lemma:fi}.]
Since $O_m = (C_0, T_1, C_1, T_2, C_2, \dots, T_m, C_m)$, Property~\ref{property:chain_rule} implies
\begin{align*}
\cI_{O_m}(N) &= \cI_{C_0}(N)  + \cI_{T_1|C_0}(N) + \cI_{C_1|T_1,C_0}(N) + \cI_{T_2|C_1,T_1,C_0}(N) +  \cI_{C_2|T_2,C_1,T_1,C_0}(N) + \dots.
\end{align*}
$\cI_{C_0}(N)=0$  since $C_0$ is a known quantity.

Note that for any $k$, $C_k$ and $T_k$ only depend on $C_{k-1}$.
Indeed, since $C_{k-1}$ determines $E_{k-1}$,
$C_k \sim \Bern\{\eta(N, \beta, C_{k-1})\}$ if $E_{k-1}$ holds and $C_k = C_{k-1}$ otherwise.
Similarly, $T_k \sim \Exp\{\lambda(N, \beta, C_{k-1})\}$ if $E_{k-1}$ holds and $T_k = \infty$ otherwise.
Therefore, we can use Property~\ref{property:indep} to simplify the above equation to
\begin{align*}
\cI_{O_m}(N) &=\sum_{k=1}^m (\cJ_{C_k|C_{k-1}}(N) + \cJ_{T_k|C_{k-1}}(N)).
\end{align*}
If $E_{k-1}=0$ (the stopping time has passed), $C_k$ and $T_k$ are deterministic conditioned on $C_{k-1}$, which implies the
score in this case is 0 (Property~\ref{property:deterministic}).
Therefore, we can condition on $E_{k-1}=1$ to write
\begin{align*}
\cI_{O_m}(N)
&= \sum_{k=1}^m \bE[g_{C_k|C_{k-1}}(C_k,C_{k-1}, N) + g_{T_k|C_{k-1}}(T_k,C_{k-1}, N)| E_{k-1}=1] \Pr(E_{k-1}=1).
\end{align*}
When $E_{k-1}=1$, the distributions of $C_k$ and $T_k$ conditioned on $C_{k-1}$ have a simple form: they are Bernoulli and exponential distributions respectively with parameters that are functions of $\beta, \gamma, N$, and $C_{k-1}$.
Evaluating the score with these distributions results in the desired equation \eqref{eq:exactFI} (see Appendix for algebra).
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lem:highprob}]
We define another infection process that has a slower rate of transmission than the SIR process of interest and is also simpler to analyze.
Let $\{A_k\}_{k =0, 1, \dots}$ be a stochastic process with stopping time $\tau_A$. % , which we define similarly to the process $\{C_k\}_{k =0, 1, \dots}$.
% Recall that if the stopping time hasn't been reached by $k-1$ jumps, $C_k - C_{k-1}\sim  \Bern(\eta(N, \beta, \gamma, C_{k-1}))$.
$\{A_k\}_k$ is defined to have the same initial condition and stopping criterion as $\{C_k\}_k$, but before the stopping time, $A_k - A_{k-1} \sim \Bern(p)$ for a constant $p$, where $p < \frac{\beta S_{k-1}}{\beta S_{k-1} + N\gamma}$ for all $k < m$.
We show $\Pr(\tau < m) \leq \Pr(\tau_A < m)$ by proving that $A_k$ is stochastically less than $C_k$ for any $k$.
Since $A_k$ is a sum of i.i.d. Bernoulli random variables up to the stopping point, $\Pr(\tau_A < m)$ can be bounded using a Chernoff bound.
\end{proof}

